Revisiting the Markov Property for Machine Translation

In this paper, we re-examine the Markov property in the context of neural machine translation. We design a Markov Autoregressive Transformer~(MAT) and undertake a comprehensive assessment of its performance across four WMT benchmarks. Our findings indicate that MAT with an order larger than 4 can generate translations with quality on par with that of conventional autoregressive transformers. In addition, counter-intuitively, we also find that the advantages of utilizing a higher-order MAT do not specifically contribute to the translation of longer sentences.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

% \jjcomment{In general, this section is missing references. For many statements, there should be relevant references to back your claims. I've added more specific comments below regarding this.}

% markov models
% causal lm are better
% we wanna question, long distance dependency.
% x, machine translation, why markov may work
% we deigsn a model, we raise question, and the findings.


Autoregressive transformer models have become the de-facto architecture for many natural language generation tasks~\cite{transformer, OpenAI2023GPT4TR}, including machine translation.
% They generate tokens one by one, conditional on all previous tokens. 
% In other words, they decompose the joint probability of a sequence of tokens into the product of conditional probabilities. 
Despite their state-of-the-art performance, 
\jjtext{a drawback of autoregressive transformers is that the model has to attend to \emph{all} previous tokens when generating the next token, which can be computationally expensive when the sequence is long.
}
% they are often criticized for the autoregressive nature, as they are fully dependent on previous tokens.
% \jjcomment{The last sentence should be further elaborated a bit (why dependency on previous tokens is not good) and needs to be backed by references.}

\jjtext{
One way to reduce the computational cost is to attend to only the previous $k$ tokens instead.
This is the Markov assumption about human languages that has been widely adopted in NLP in the past such as in $n$-gram language models.
Compared with autoregressive transformers attending to all previous tokens, supposedly Markov models lose the ability to model long-range dependencies and therefore may deliver lower performance.
% Compared with Markov models, autoregressive transformers attending to all previous tokens have the advantage of modeling long-range dependencies.
However, to the best of our knowledge, there has not been any previous work studying how critical long-range dependencies are for neural machine translation.
In other words, for machine translation, if we make the Markov assumption and have the transformer attending to only the previous $k$ generated tokens as well as the encoded input tokens during decoding, would the translation performance be significantly affected?
In this paper, we design a Markov Autoregressive Transformer~(MAT) and empirically compare its performance with that of the vanilla autoregressive transformer to answer this research question.
}

\jjtext{
It may be worth noting that exploiting the Markov property for machine translation has been explored in some recent work.
\citet{natcrf} proposed an NART-CRF model that combines non-autoregressive machine translation with a linear-chain conditional random field~(CRF) model (which makes a 1st order Markov assumption) to capture the local dependency between adjacent tokens.
\citet{Deng2020Cascadedmarkovnat} proposed a similar idea but considered higher-order Markov models.
They applied a cascaded decoding strategy to iteratively incorporate higher-order dependencies into the output of a non-autoregressive model.
Different from these studies, our Markov transformer model is used within an autoregressive framework.
More importantly, we note that the two studies mentioned above achieved subpar translation performance compared with autoregressive models, which may suggest that their relatively low performance is due to Markov models' inability to capture long-range dependencies.
However, as we will show in Section~\ref{}, our Markov transformer applied in an autoregressive setting is highly competitive with a vanilla autoregressive transformer, which indicates that the Markov assumption itself is not the main cause of the relatively low translation performance of the two models above.
}

\jjtext{
Specifically, our Markov Autoregressive Transformer model employs a simple modification to the causal mask in the decoding stage.
We also introduce a ``transparent attention'' mechanism to ensure the Markov property.
This transparent attention mechanism also reduces the need to cache the contextualized embeddings of the previous tokens.
With this modification, during training, our model can still be parallelized, just like vanilla autoregressive transformers.
It is also worth pointing out that our Markov Autoregressive Transformer is different from the Markov transformer architecture proposed by \citet{Deng2020Cascadedmarkovnat}, which we will explain in detail in Section~\ref{}.
}

\jjtext{
Our experiments on several MT benchmarks comparing out Markov Autoregressive Transformer and vanilla autoregressive transformer show that although with a first-order Markov assumption, the translation performance is substantially impaired, with higher orders of Markov assumptions, the performance of the our MAT model becomes increasingly comparable to that of a vanilla autoregressive model.
We also find that longer input sentences do not necessarily require larger values of $k$.
}

\cxdu{do we need to introduce more details here}
\jjcomment{I don't think we need more details here.}



% To answer this question we first introduce a Markov Autoregressive Transformer (MAT) which  
% To model the transition among the current token and previous $k$ tokens, a common solution is to adopt a matrix with the size of $(|V|, |V|, ..., |V|)$, where $V$ denotes the set of candidate tokens, e.g., sec-order CRF in neural dependency parsing~\cite{Zhang2020secordercrf}.

% Obviously, these Markov models only work for tasks with limited $|V|$, e.g., semantic role parsing. 
% For the task like machine translation, which has a candidate size of 32K and more, it will be a disaster to compute or store the transition matrix. 
% Additionally, the huge amount of $|L|$ also restricted the choice of $k$. So the classical Markov models are seldom used for the generation task, e.g., machine translation.


% To overcome the huge transition matrix problem, we propose a new Markov Autoregressive Transformer (MAT). Which could transfer the transition matrix into the parameters of the transformer instead of directly explicitly storing them. Specifically, we use a transformer model to encode the previous k tokens, i.e., $Transformer([y_{n-k}, y_{n-k + 1}, \cdots, y_{n-1}])$, and output a probability distribution over the label set. In this context, we cannot directly use the transformer model with a previous attention mask to build MAT, as dependencies can be conveyed through the attention values. Specifically, for a first-order MAT, token 5 cannot obtain any information from token 3. However, in reality, token 5 can obtain a representation of token 3 by attending to the value of token 4. This is because, when token 4 attends to token 3, its value already includes information from token 3. This indicates that simple masking might not be sufficient to enforce the Markov property. So we further modified the attention to contextless attention to make sure the Markov property.

% However, MAT still needs to run the model $|V|^k$ times to get the transition matrix. To avoid this, we propose optimizing the local normalized MAT instead of the global normalization. Even though local normalization inevitably compromises the performance, we have successfully transformed an unoptimizable problem into one that can be optimized. Moreover, the empirical evaluation demonstrated that compared to global normalization, a parameterized dynamic transition matrix is more worthwhile. Local normalization also empowers training parallelism like the vanilla transformer to fully utilize GPU.



% From the view of autoregressive Model
% ngram LM
% Additionally, our method also raises the question of whether the Markov property is indeed a favorable trade-off between performance and speed for a powerful translation model like the transformer. Contrary to the intricate full history tokens dependencies observed in open-ended text generation, machine translation exhibits a commendable adherence to the Markov property when confronted with a given source sentence. 

% From the view of CRF
% \jjcomment{This paragraph maybe can be moved to the end as part of the discussions.} Meanwhile, our work also calls for rethinking the design and optimization of the Markov model. Classical Markov models are usually global normalization (i.e., normalization over all the possible sequences), which is treated as one of the main advantages, while it also prevents high-order interaction, deep interaction between tokens, and usage of large label set tasks. Our MAT discards global normalization and chooses the local one, which significantly reduces the training complexity and also boosts performance by a large margin.


==> intro_v0.tex <==
\section{Introduction (version 0)}

\jjcomment{The paragraphs below are moved here from the original intro section.}

Recently, other approaches relying on Markov property have been introduced to accelerate autoregressive transformers. 
\jjcomment{The previous sentence may cause criticism because the acceleration achieved in the two papers below comes mostly from parallelization, as I understand it.}
\citet{natcrf} propose using a Conditional Markov Random Field~(CRF) to accelerate the autoregressive transformer and ~\citet{Deng2020Cascadedmarkovnat} use cascaded Markov transformers to generate the output sequence in parallel. These models utilize the Markov property to lower the complexity, i.e.,  the generation of the $n$-th token is dependent on only the previous $k$ tokens rather than the previous $(n-1)$ tokens. Despite the speed improvements achieved by these models, it comes at the expense of model performance. For example, the CRF model~\cite{natcrf} underperformed the standard autoregressive transformer by a margin of 4.1 BLEU points on the WMT14 EN-DE.

The discrepancy between Markov models and the standard autoregressive transformer has piqued our interest. 
Especially considering that Markov models often also rely on the transformer architecture with similar parameters as the autoregressive one, \jjcomment{If you say that Markov models \emph{often} also rely on the transformer architecture, what kind of Markov models are you referring to? I don't think we can claim that they're \emph{often} relying on transformer architecture, because we haven't seen many Markov transformer models, right?} \cxdu{yes prof, the point i want to say is the current two markov translation models are based on transformer} which suggests that the difference is not attributed to the neural network structure itself. 
An intuition might be that the Markov property prevents the decoder from capturing long-distance dependencies, which in turn might degrade the performance. 
Unfortunately, although a lot of work on the Markov model has been done, the question of how the impact of Markov property in the MT system remains unexplored. In this paper, we aim to address this research question, and further investigate the performance limits of Markov models.

\jjcomment{It seems to me that this paragraph is mainly saying that our MAT uses a simple modification to the causal mask to achieve Markov property. Are there any other major points?} \cxdu{may be embedding attention is the other one ?} To address this issue, we introduce the Markov Autoregressive Transformer (MAT). MAT possesses two main features: 1) minimal modifications compared to the autoregressive transformer, and 2) support for high-order Markov models. Specifically, the key idea of the k-order Markov property is that the next output token by the model is only dependent on the previous k words. We discovered that this objective can be achieved with a simple modification to the causal mask in the decoder part. In contrast to previous Markov models, this simple modification ensures that MAT has only marginal alterations compared to the autoregressive transformer. This allows us to effectively isolate and examine the effects of Markov property in a manner akin to a controlled variable experiment. In addition to the aforementioned benefit, this straightforward modification also enables us to train MAT in parallel, like the vanilla transformer.


We evaluate MAT on several WMT benchmarks and find the following observations:
\begin{itemize}
    \item The first-order Markov property significantly impairs model performance. For instance, on the WMT14 EN-DE task, there is a decline of approximately 3.4 BLEU points~(\S \ref{sec: }).
    \item For the $k$-order Markov property, as $k$ increases, the performance of the model becomes increasingly comparable to that of an autoregressive model (e.g., when k=5)~(\S \ref{sec: }).
    \item Longer sentences do not necessarily require larger values of $k$. The benefits of a larger $k$ are not necessarily specific to longer sentences~(\S \ref{sec: }).
\end{itemize}


In addition to the aforementioned findings, we also discovered that MAT also enjoys the following advantages: 1) Linear complexity of attention. To generate a sentence with the length of $n$, the complexity of attention is only $O(kn)$ compared with $O(n^2)$ in vanilla AT. This results in over a 3-fold reduction in computational cost for self-attention calculation at each step of the decoder.
 and 2) Key-Value cache free inference. Because MAT only attends to the embeddings of the previous $k$ tokens, our model does not require caching any keys and values of previous tokens during inference. This reduces the memory bandwidth required by the cache at the decoding stage. 
 By limiting the dependence on a fixed number of preceding tokens, the Markov property can potentially simplify the translation model, thereby reducing complexity and computational requirements. 
This might lead to a balance where adequate performance can be achieved more efficiently.




\jjcomment{This paragraph maybe can be moved to the end as part of the discussions.} Meanwhile, our work also calls for rethinking the design and optimization of the Markov model. Classical Markov models are usually global normalization (i.e., normalization over all the possible sequences), which is treated as one of the main advantages, while it also prevents high-order interaction, deep interaction between tokens, and usage of large label set tasks. Our MAT discards global normalization and chooses the local one, which significantly reduces the training complexity and also boosts performance by a large margin.

==> related.tex <==
\section{Related Work}

Markov models leverage the Markov assumption to model sequences in the output space, striking a balance between capturing the dependencies between outputs and minimizing the computational complexity. These models have found extensive applications in natural language processing (NLP), a notable example is the conditional random fields (CRF)~\cite{Lafferty2001ConditionalRF}.
%ner and parsing
In the context of named entity recognition (NER), Ling and Weld (2012) employed linear-chain CRF to extract entity mentions. Further pushing the boundaries, Jie et al. (2017) proposed a dependency-guided approach, capitalizing on the semi-Markov CRF~\cite{Sarawagi2004SemiMarkovCR} for enhanced NER performance. In the field of parsing, ~\citet{Durrett2015NeuralCP} proposed a neural CRF parser with rich nonlinear featurization from the neural network. 

The usage of Markov property has also been explored in machine translation. The CRF-based approaches in Statistical Machine Translation (SMT) can be attributed to the pioneering work ~\cite{Lavergne2011smtcrf}. With the rise of neural machine translation, researchers have increasingly chosen autoregressive models over Markov models. However, recent attention has been drawn to the fact that Markov property can aid in non-autoregressive generation. ~\citet{natcrf} proposed using Conditional Random Fields (CRF) for fast translation, while ~\citet{Deng2020Cascadedmarkovnat} suggested the use of cascade Markov models to further model higher-order Markov relationships. Compared to autoregressive models, these neural CRFs have achieved significant improvements in inference speed, but at the cost of considerably sacrificed performance. Unlike their research, which primarily focuses on speed enhancement, we aim to investigate whether satisfying Markov property would compromise model performance.
